A Tableau Method for the Realizability and Synthesis of Reactive Safety Specifications

We introduce a tableau decision method for deciding realizability of specifications expressed in a safety fragment of LTL that includes bounded future temporal operators. Tableau decision procedures for temporal and modal logics have been thoroughly studied for satisfiability and for translating temporal formulae into equivalent B\"uchi automata, and also for model checking, where a specification and system are provided. However, to the best of our knowledge no tableau method has been studied for the reactive synthesis problem. Reactive synthesis starts from a specification where propositional variables are split into those controlled by the environment and those controlled by the system, and consists on automatically producing a system that guarantees the specification for all environments. Realizability is the decision problem of whether there is one such system. In this paper we present a method to decide realizability of safety specifications, from which we can also extract (i.e. synthesize) a correct system (in case the specification is realizable). Our method can easily be extended to handle richer domains (integers, etc) and bounds in the temporal operators in ways that automata approaches for synthesis cannot.

==> preliminaries.tex <==
\section{Preliminaries}
\label{sec:prelims}

Linear Temporal Logic (\ltl)~\cite{pnueli77temporal}, extends
propositional logic by introducing temporal operators $\Next$ (next)
and $\Until$ (until).
%
\ltl formulas are interpreted in traces on their set of (occurring) variables $\MV$.
A {\it trace} $\sigma$ is a denumerable sequence of states $\sigma_0,\sigma_1,\sigma_2,\dots$ where each state $\sigma_i$ is a valuation from $\MV$ to $\{0,1\}$. 
A valuation $v$ on a set of variables $\MV$ is a function that assigns to each $p\in\MV$ a boolean value $\{0,1\}$. We denote by $\Val(\MV)$ the set of all valuations on $\MV$.
For any $i\geq 0$, $\sigma^i$ denotes the trace $\sigma_i,\sigma_{i+1},\dots$ and $\sigma^{<i}$ denotes the finite sequence
$\sigma_0,\dots,\sigma_{i-1}$. Therefore, $\sigma = \sigma^{<i}\cdot\sigma^i$. We also use $\sigma^{i..j}$ for the finite sequence between $i$ and $j$ (including $\sigma_i$ but not $\sigma_j$), which can be defined as $(\sigma^i)^{<j}$. 
%
Given a trace $\sigma$ and an \ltl formula $\phi$ the meaning of $\sigma\models \phi$ is  inductively defined as follows:
%
\[
\begin{array}{lcl}
\sigma \models p  &\mbox{ iff } & \sigma_0(p) = 1\\
\sigma\models\neg\phi &\text{iff} & \sigma\not\models\phi\\
\sigma\models \phi\And\psi &\text{iff}& \sigma\models\phi \mbox{ and } \sigma\models\psi \\
\sigma \models\Next \phi    &\mbox{ iff }& 
\sigma^{1} \models \phi.\\ 
 \sigma\models \phi\Until\psi  &\mbox{ iff } &
  \sigma^j \models \psi  \textrm{ for some } j  \textrm{ such that }  0 \leq j \textrm{ and } \\ 
  & & \sigma^i \models \phi  \textrm{ for all } i  \textrm{ such that }  0 \leq i < j.
\end{array}
\]

%
There are standard abbreviations of constants propositions ($\cT$ for truth and $\cF$ for falsehood), classical connectives (such as $\vee,\Impl$ and $\Iff$) and also of temporal operators such as `eventually': $\Eventually \phi$ for $\cT\Until\phi$ and `always': $\Always\phi$ for
$\Not(\cT\Until\Not\phi)$.

%
A set of formulas is (syntactically) consistent if and only if it does not contain a formula and its negation.
%
If $\sigma\models \phi$ then  we say that $\sigma$ models (or is a model of) $\phi$.
We denote $\Mod(\phi)$ to the set of all traces that are models of $\phi$.
Finite set of formulas are intentionally confused with the conjunction of all it members. Therefore, for a set of formulas $\Phi$, $\sigma\models\Phi$ if and only if $\sigma\models\phi$ for all $\phi\in\Phi$ and $\Mod(\Phi)$ denotes the set of traces that are models of all $\phi\in\Phi$.
%
A set of formulas $\Phi$ is satisfiable if and only if there exists at least one $\sigma$ such that $\sigma\models\Phi$, otherwise $\Phi$ is unsatisfiable. Two formulas $\phi$ and $\psi$ are logically equivalent, denoted $\phi\equiv\psi$, if and only if $\Mod(\phi) = \Mod(\psi)$.

%
% Safety LTL
Any sublanguage $\mathcal{G}$ of LTL is {\it safety} whenever for any formula $\phi\in\mathcal{G}$  and for any trace $\sigma$, if $\sigma\not\models\phi$ then there exists some $i > 0$ such that $\sigma^{<i}\cdot\sigma'\not\models\phi$ for any trace $\sigma'$. In words,  any trace with prefix $\sigma^{<i}$ is not a model of $\phi$. In such case, $\sigma^{<i}$ is called a {\it witness of the violation} of $\phi$ (a.k.a. a {\it bad prefix} for $\phi$).

%%% Local Variables:
%%% TeX-master: "main.tex"
%%% TeX-PDF-mode: t
%%% End:

